EO-Agents: A Three-Agent LLM Pipeline for Earth Observation Hypothesis Generation

Large language models have recently been explored for scientific hypothesis generation, but most prior work relies on unstructured literature and free-form textual claims. We present a pipeline for Earth observation that grounds hypothesis generation directly in the NASA Earth Observation Knowledge Graph. A heterogeneous graph neural network trained on historical co-usage relations ranks candidate dataset pairings, and a three-agent LLM pipeline filters, generates, and evaluates structured research hypotheses. Applied to 1,475 NASA datasets, the system produces 160 hypotheses spanning multiple Earth-science domains, including ecohydrology, glaciology, aerosol--cloud interactions, vegetation phenology, and stratospheric chemistry. Model-predicted novel dataset pairings are rated nearly as plausible as held-out real co-usages from the literature, indicating that the pipeline surfaces scientifically coherent yet unexplored combinations. A 2*2*2 factorial experiment across GPT-5.2 and Claude Sonnet 4.6 shows that hypothesis rankings remain stable, while absolute scores depend strongly on judge identity, highlighting limitations of single-judge LLM evaluation.

==> figures/neurips_tables_only.tex <==
% ════════════════════════════════════════════
% NASA EO Knowledge Graph — Paper Tables
% Generated by stage0_pipeline.py (from live GraphML)
% ════════════════════════════════════════════
% Required packages: booktabs, siunitx, xcolor

\begin{table}[t]
\centering
\caption{Summary statistics of the NASA Earth Observation Knowledge Graph (NASA EO-KG), computed directly from the released GraphML.}
\label{tab:graph_stats}
\small
\begin{tabular}{lrr}
\toprule
\textbf{Property} & \textbf{Value} & \textbf{Note} \\
\midrule
Total nodes       & \num{150351}   & 7 distinct types \\
Total edges       & \num{436203}   & 9 relation types \\
Mean degree       & 5.80           & Across all nodes \\
Max degree        & \num{41110}       & High-citation node \\
Publications      & \num{138704} & 99.5\% with title/abstract \\
Datasets          & \num{8058} & 100\% with CMR metadata \\
Dataset temporal span & 1972–2026 & Earliest start -- latest end \\
CITES edges       & \num{208616}   & Citation network \\
USES\_DATASET     & \num{44354}   & Pub.\ $\to$ Dataset links \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Node type distribution in NASA EO-KG with key attributes.}
\label{tab:node_types}
\small
\begin{tabular}{llrp{4.5cm}}
\toprule
\textbf{Node Type} & \textbf{Count} & \textbf{\%} & \textbf{Key Attributes} \\
\midrule
\texttt{Publication} & \num{138704} & 92.3\% & doi, title, year, authors, abstract \\
\texttt{Dataset} & \num{8058} & 5.4\% & shortName, longName, daac, cmrId, temporal extent \\
\texttt{ScienceKeyword} & \num{1609} & 1.1\% & name, subcategory hierarchy \\
\texttt{Instrument} & \num{921} & 0.6\% & shortName, longName \\
\texttt{Platform} & \num{455} & 0.3\% & shortName, longName, Type \\
\texttt{Project} & \num{415} & 0.3\% & shortName, longName \\
\texttt{DataCenter} & \num{189} & 0.1\% & shortName, longName, url \\
\midrule
\textbf{Total} & \num{150351} & 100\% & \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Edge (relation) types in NASA EO-KG with dominant source and target node types.}
\label{tab:edge_types}
\small
\begin{tabular}{llll r}
\toprule
\textbf{Relation} & \textbf{Source} & \textbf{Target} & \textbf{Count} & \textbf{\%} \\
\midrule
\texttt{CITES} & \texttt{Publication} & \texttt{Publication} & \num{208616} & 47.8\% \\
\texttt{HAS\_APPLIEDRESEARCHAREA} & \texttt{Publication} & \texttt{ScienceKeyword} & \num{121553} & 27.9\% \\
\texttt{USES\_DATASET} & \texttt{Publication} & \texttt{Dataset} & \num{44354} & 10.2\% \\
\texttt{HAS\_SCIENCEKEYWORD} & \texttt{Dataset} & \texttt{ScienceKeyword} & \num{25553} & 5.9\% \\
\texttt{HAS\_PLATFORM} & \texttt{Dataset} & \texttt{Platform} & \num{11944} & 2.7\% \\
\texttt{HAS\_DATASET} & \texttt{DataCenter} & \texttt{Dataset} & \num{11698} & 2.7\% \\
\texttt{OF\_PROJECT} & \texttt{Dataset} & \texttt{Project} & \num{8031} & 1.8\% \\
\texttt{HAS\_INSTRUMENT} & \texttt{Platform} & \texttt{Instrument} & \num{2631} & 0.6\% \\
\texttt{HAS\_SUBCATEGORY} & \texttt{ScienceKeyword} & \texttt{ScienceKeyword} & \num{1823} & 0.4\% \\
\midrule
\textbf{Total} & & & \num{436203} & 100\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Distribution of NASA EO-KG datasets across Distributed Active Archive Centers (DAACs).}
\label{tab:daac}
\small
\begin{tabular}{llr r}
\toprule
\textbf{DAAC} & \textbf{Full Name} & \textbf{Datasets} & \textbf{\%} \\
\midrule
\texttt{ASDC} & Atmospheric Science Data Center & \num{1601} & 19.9\% \\
\texttt{GES-DISC} & Goddard Earth Sciences DISC & \num{1450} & 18.0\% \\
\texttt{LP DAAC} & Land Processes DAAC & \num{966} & 12.0\% \\
\texttt{NSIDC} & Natl.\ Snow and Ice Data Center & \num{889} & 11.0\% \\
\texttt{PODAAC} & Physical Oceanography DAAC & \num{846} & 10.5\% \\
\texttt{OB.DAAC} & Ocean Biology DAAC & \num{677} & 8.4\% \\
\texttt{GHRC} & Global Hydrology Resource Ctr. & \num{639} & 7.9\% \\
\texttt{Other} & Remaining DAACs & \num{990} & 12.3\% \\
\midrule
\textbf{Total} & & \num{8058} & 100\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Co-usage statistics for the NASA EO-KG. Co-usage edges are dataset pairs cited together in at least one publication. Train/Val/Test split is temporal (pre-2023 / 2023 / 2024).}
\label{tab:cousage_stats}
\small
\begin{tabular}{lr}
\toprule
\textbf{Property} & \textbf{Value} \\
\midrule
Paper$\to$Dataset edges (total)       & \num{44354} \\
Unique datasets cited                  & \num{2357} \\
Datasets with $\geq 5$ papers         & \num{949} \\
Papers citing $\geq 2$ datasets       & \num{11087} \\
\midrule
Co-usage graph nodes                   & \num{2088} \\
Co-usage graph edges (unique pairs)    & \num{23490} \\
Sum of co-usage weights                & \num{64930} \\
Max pair weight                        & \num{1051} \\
Median / Max degree                    & 11 / \num{314} \\
\midrule
Train co-usage pairs                   & \num{13529} \\
Val co-usage pairs                     & \num{6119} \\
Test co-usage pairs                    & \num{6319} \\
Test pairs unseen in train             & \num{3944} \\
\midrule
Cold-start test pairs                  & \num{2284} \\
Cross-DAAC test pairs                  & \num{1480} \\
Cross-instrument test pairs            & \num{902} \\
\bottomrule
\end{tabular}
\end{table}


==> figures/tab_inter_rater.tex <==
\begin{table}[h]
\centering
\small
\caption{Inter-rater agreement between GPT-5.2 and Claude Sonnet 4.6 on identical hypotheses. Judges agree best on tractability (Pearson $r > 0.60$), less on novelty, and only weakly on importance ($r \approx 0.35$–$0.40$). Showing full dataset context improves agreement on all three axes. $\kappa_q$ is Cohen's quadratic-weighted kappa.}
\label{tab:inter_rater}
\begin{tabular}{llccccc}
\toprule
Axis & Condition & $n$ & Pearson $r$ & Spearman $\rho$ & $\kappa_q$ & Exact \% \\
\midrule
Importance & blind & 160 & +0.351 & +0.337 & +0.137 & 37 \\
Importance & ctx & 160 & +0.397 & +0.366 & +0.241 & 63 \\
Tractability & blind & 160 & +0.627 & +0.578 & +0.472 & 54 \\
Tractability & ctx & 160 & +0.601 & +0.585 & +0.572 & 58 \\
Novelty & blind & 160 & +0.487 & +0.456 & +0.356 & 57 \\
Novelty & ctx & 160 & +0.527 & +0.541 & +0.512 & 71 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/tab_stage4_strata.tex <==
\begin{table}[h]
\centering
\small
\caption{Stage 4 pair-level judgments. Each of 800 pairs (200 per stratum) was scored by both GPT-5.2 and Claude Sonnet 4.6 on plausibility and novelty (1–5). Both judges order the strata identically (B $\geq$ A $>$ D $>$ C on plausibility); Claude's scores show a tighter distribution on novelty but a larger A$-$C plausibility gap.}
\label{tab:stage4_strata}
\begin{tabular}{llcccc}
\toprule
\multirow{2}{*}{Stratum} & \multirow{2}{*}{Description} & \multicolumn{2}{c}{Plausibility} & \multicolumn{2}{c}{Novelty} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
& & GPT-5.2 & Claude 4.6 & GPT-5.2 & Claude 4.6 \\
\midrule
B & Held-out real co-usages (2024) & 4.57 & 4.63 & 2.35 & 1.86 \\
A & Predicted novel (model top-ranked) & 4.38 & 4.34 & 2.19 & 1.84 \\
D & Hard negatives (same-DAAC novel) & 3.66 & 3.46 & 3.17 & 2.48 \\
C & Random novel pairs & 3.31 & 2.75 & 3.52 & 2.75 \\
\bottomrule
\end{tabular}
\end{table}
